Words into Action: Learning Diverse Humanoid Robot Behaviors using Language Guided Iterative Motion Refinement

Humanoid robots are well suited for human habitats due to their morphological similarity, but developing controllers for them is a challenging task that involves multiple sub-problems, such as control, planning and perception. In this paper, we introduce a method to simplify controller design by enabling users to train and fine-tune robot control policies using natural language commands. We first learn a neural network policy that generates behaviors given a natural language command, such as "walk forward", by combining Large Language Models (LLMs), motion retargeting, and motion imitation. Based on the synthesized motion, we iteratively fine-tune by updating the text prompt and querying LLMs to find the best checkpoint associated with the closest motion in history. We validate our approach using a simulated Digit humanoid robot and demonstrate learning of diverse motions, such as walking, hopping, and kicking, without the burden of complex reward engineering. In addition, we show that our iterative refinement enables us to learn 3x times faster than a naive formulation that learns from scratch.

==> humaoid_related_work.tex <==
A natural solution to building robots adapted to the human living environment, is to adopt a morphology similar to human form. 
However, designing controllers for humanoid robots that are versatile and robust to external perturbations is a challenging problem that has been studied extensively over the last few decades. A classical approach is to develop a dynamics model for the robot and then use it to develop controllers that plan and execute control actions, optimizing a specified objective. These models~\cite{grizzle2014models,hurmuzlu2004modeling} span from simple approximations that reduce the robot to a linear inverted pendulum~\cite{raibert1986legged,kajita2003biped, yamaguchi1999development, sugihara2002real,hirai1998development} to more sophisticated alternatives that consider the entire dynamics of the humanoid~\cite{posa2016optimization, henze2015approach} or some combination of the two strategies~\cite{dai2014whole}. While simpler models make the problem tractable from a computational standpoint, they sacrifice exploiting the full capabilities of the robot dynamics and constrain themselves to motion feasible on the simple model. Modeling the full dynamics of the robot, on the other hand, is difficult and time-consuming and may not be applicable for real-time robot control. 
% Over the recent years, learning based approaches have emerged to become an attractive alternative to model-based control.

In recent years, learning-based approaches, particularly deep reinforcement learning (DRL)~\cite{sutton2018reinforcement} have gained increasing attention from the humanoid robot control community, following impressive results on quadruped~\cite{tan2018sim,lee2020learning} and bipedal robots~\cite{li2021reinforcement,kumar2022adapting}.
Some work incorporates learning within other model-based frameworks to improve robustness and adaptability. For example, in~\cite{castillo2022reinforcement} a learned policy generates actuator trajectories that are then tracked using a feedback regulator designed with the robot model. In a related work~\cite{krishna2022linear}, a learned policy acts as a foot-trajectory modulator while a low-level gait controller regulates the torso and ankle orientation.
But a more recent line of work takes an end-to-end learning-based framework to develop humanoid robot controllers~\cite{radosavovic2023learning,guo2023decentralized}. Unlike model-based approaches, learning based techniques do not require solving for the control output at every time-step using the robot dynamics model, which makes them suitable for high-frequency real-time control. These policies can be trained in massively parallelized simulations~\cite{makoviychuk2021isaac} and transferred directly to the real-world without any additional fine-tuning. 
While learning-based approaches offer a powerful alternative to model-based control, it is often challenging to design and tune reward functions to accomplish a given task. Recent work,~\cite{escontrela2022adversarial,peng2020learning} leverages expert demonstrations to ground the space of behaviors that emerge from the policy by imposing a motion prior.
